RescoreBERT: Discriminative Speech Recognition Rescoring with BERT

Second-pass rescoring is an important component in automatic speech recognition (ASR) systems that is used to improve the outputs from a first-pass decoder by implementing a lattice rescoring or $n$-best re-ranking. While pretraining with a masked language model (MLM) objective has received great success in various natural language understanding (NLU) tasks, it has not gained traction as a rescoring model for ASR. Specifically, training a bidirectional model like BERT on a discriminative objective such as minimum WER (MWER) has not been explored. Here we show how to train a BERT-based rescoring model with MWER loss, to incorporate the improvements of a discriminative loss into fine-tuning of deep bidirectional pretrained models for ASR. Specifically, we propose a fusion strategy that incorporates the MLM into the discriminative training process to effectively distill knowledge from a pretrained model. We further propose an alternative discriminative loss. This approach, which we call RescoreBERT, reduces WER by 6.6%/3.4% relative on the LibriSpeech clean/other test sets over a BERT baseline without discriminative objective. We also evaluate our method on an internal dataset from a conversational agent and find that it reduces both latency and WER (by 3 to 8% relative) over an LSTM rescoring model.

==> tab/mlm.tex <==
\begin{table}[htbp!]
\centering
\caption{Evaluation results using BERT with two settings of LM scoring (Section~\ref{subsec:mlm-result}). \texttt{TC}/\texttt{TO}: Test-Clean/Other for LibriSpeech. \texttt{IE}/\texttt{IJ}/\texttt{NJ}: Info (en), Info (ja), Navigation (ja).}
\label{tab:mlm}
\resizebox{0.71\columnwidth}{!}{
\begin{tabular}{l|cc|ccc}
\toprule
& \tt TC & \tt TO & \tt IE & \tt IJ & \tt NJ \\
\midrule
PLL & 4.54 & 16.08 & 4.3\% & 5.8\% & 4.4\% \\
MD & 4.67 & 16.15 & 2.6\% & 3.7\% & 5.6\% \\
\; -17M & - & - & 2.9\% & 1.7\% & 1.6\% \\
\bottomrule
\end{tabular}}
\vspace{-0.5ex}
\end{table}


==> tex/related.tex <==
\section{Related Work}
\label{sec:related}
